Model Checking Probabilistic Pushdown Automata

We consider the model checking problem for probabilistic pushdown automata (pPDA) and properties expressible in various probabilistic logics. We start with properties that can be formulated as instances of a generalized random walk problem. We prove that both qualitative and quantitative model checking for this class of properties and pPDA is decidable. Then we show that model checking for the qualitative fragment of the logic PCTL and pPDA is also decidable. Moreover, we develop an error-tolerant model checking algorithm for PCTL and the subclass of stateless pPDA. Finally, we consider the class of omega-regular properties and show that both qualitative and quantitative model checking for pPDA is decidable.

==> xypdftex.tex <==
%% xypdftex.tex from $Id: xypdftex.doc,v $
%%
%% Xy-pic ``pdf-TeX'' driver interface option.
%% Copyright (c) 1999-1999 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{pdftex}{pdf-TeX driver}{\stripRCS$Revision: 3.8 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\pdfTeX@@#1{\dvimessage@{pdf-TeX}{#1}}
\newdriver{%
 \xyaddsupport{color}\pdftexColor@@
 \xyaddsupport{crayon}\pdftexCrayon@@
% \xyaddsupport{pdf}\pdftexPDF@@
% \xyaddsupport{rotate}\pdftexRotate@@
 \xyaddsupport{line}\pdftexLine@@
% \xyaddsupport{frame}\pdftexFrames@@
% \xyaddsupport{tile}\pdftexTiles@@
 \xyaddsupport{cmtip}\relax
}
%\xydef@\pdfTeXcolor@push#1{\special{pdfcolor push}\special{pdfcolor #1}}
\xydef@\pdfTeXcolor@push#1{\edef\pdfsaved@color{\pdfcurrent@color}%
 \def\pdfcurrent@color{#1}\special{#1}}%%%<<<<<<--- WRONG !
\xydef@\pdfTeXcolor@pop{\let\pdfcurrent@color\pdfsaved@color
 \expandafter\special\expandafter{\pdfsaved@color}}
\xydef@\pdfTeXcolours@{\pdftexPDFtypes@
% \let\xylocalColor@=\xystackcolor@
% \let\xycolor@push=\pdfTeXcolor@push
% \let\xycolor@pop=\pdfTeXcolor@pop
 \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-c}{\xydrivernoload@{pdf-c}}%
 \if@pdf@known\installPDFcolor@ }\else\DN@{}\fi \next@
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\pdftexCrayon@@{}}%
 \else\let\next@=\xystandardcolors@ \fi \next@ 
 \let\xycolorwarning@=\relax \pdfTeX@@{color}%
 \let\pdftexColor@@=\relax
 \let\UnloadColor@@=\NopdfTeXcolor@
 }
\xydef@\pdftexColor@@{\pdfTeXcolours@}
\xydef@\NopdfTeXcolor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\pdftexColor@@=\pdfTeXcolours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\pdftexCrayon@@{\pdftexColor@@\pdftexCrayon@}
\xydef@\pdftexCrayon@{\installCrayolaColors@}%
\xydef@\pdftexPDF@@{\if@pdf@known\pdftexPDF@}
\xydef@\pdftexPDFunload@{\if@pdf@known\UnloadPDF@
 \let\UnloadPDF@@=\UnloadPDF@
 \let\pdftexPDF@@=\pdftexPDF@ }
\xydef@\pdftexPDFtypes@{%
 \xyinputorelse@{xypdfpdf}{\xydrivernoload@{pdfpdf}}%
 \ifx\PDFspecial@@\pdfTeXspecial@\else
 \let\PDFspecial@@=\pdfTeXspecial@
 \let\PDFmacro@@=\pdfTeXmacro@
 \let\PDFdict@@=\pdfTeXdict@
 \let\PDFraw@@=\pdfTeXraw@
 \let\PDFinclude@@=\pdfTeXinclude@
 \let\PDFspecialdict@@=\pdfTeXspecialDict@
 \let\xyPDFobeylines@@=\obeypdfTeXlines@
 \pdfTeX@@{PDF}%
 \fi \pdftexCurrpt@ }
\xydef@\pdfTeXspecial@#1{\if@pdf@known\firstPDF@@\pdfobj{#1}\pdflastobj}
\xydef@\pdfTeXmacro@#1{\pdfobj{#1}}
\xydef@\pdfTeXdict@#1{\pdfnames{#1}}
\xydef@\pdfTeXspecialDict@#1{\pdfnames{#1}}
\xydef@\pdfTeXinclude@#1{\if@pdf@known\firstPDF@@\special{prePDFfile #1}}
\xydef@\pdfTeXraw@#1{\if@pdf@known\firstPDF@@\pdfliteral{#1}}%
{\catcode`\^^M=\active%
 \gdef\next{\catcode`\^^M=\active \let^^M=\par%
 \let\PDFspecial@@=\pdfTeXdict@ \obeyspaces}}
\xylet@\obeypdfTeXlines@=\next
\xydef@\pdftexCurrpt@{\let\xyPDFcurrpt@@=\pdftexCurrpt@@}%
\xydef@\pdftexCurrpt@@{\PDFspecial@@{xyi}\PDFraw@@{userdict begin xyx end}}%%%%%<<<<<--- here
\xydef@\pdftexPDF@{\pdftexPDFtypes@
 \let\pdftexPDF@@=\relax
 \let\UnloadPDF@@=\pdftexPDFunload@ 
 \let\installxypdf@@=\relax \if@pdf@known\installxypdf@ }
\xydef@\pdftexRotate@@{\pdftexRotate@}
\xydef@\pdftexRotate@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-r}{\xydrivernoload@{pdf-r}}%
 \xyRotScale@@ \if@pdf@known\installPDFrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}\if@pdf@known\UnloadRotate@\relax}\fi
 \next@}
\xydef@\pdftexLine@@{\pdftexLine@}
\xydef@\pdftexLine@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-l}{\xydrivernoload@{pdf-l}}%
 \if@pdf@known\installPDFline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\if@pdf@known\UnloadLine@\relax}\fi
 \next@ }
\xydef@\pdftexFrames@@{\pdftexFrames@}
\xydef@\pdftexFrames@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-f}{\xydrivernoload@{pdf-f}}%
 \if@pdf@known\installPDFframes@ }%
 \else\DN@{\xydriverfail@{frames are}\if@pdf@known\UnloadPDFframes@\relax}\fi
 \next@ }
\xydef@\pdftexTiles@@{\pdftexTiles@}
\xydef@\pdftexTiles@{\pdftexPDFtypes@
 \expandafter\ifx\csname xypdf-pdfloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xypdf-t}{\xydrivernoload@{pdf-t}}%
 \if@pdf@known\installPDFpatterns@ \xystandardpatterns@}%
 \else\DN@{\xydriverfail@{Patterns are}\if@pdf@known\UnloadPDFpatterns@\relax}\fi
 \next@ }
\xydef@\if@pdf@known#1{\ifx\undefined#1\else\expandafter#1\fi}
\xyendinput



